Evaluating Generative Language Models in Information Extraction as Subjective Question Correction

Modern Large Language Models (LLMs) have showcased remarkable prowess in various tasks necessitating sophisticated cognitive behaviors. Nevertheless, a paradoxical performance discrepancy is observed, where these models underperform in seemingly elementary tasks like relation extraction and event extraction due to two issues in conventional evaluation. (1) The imprecision of existing evaluation metrics that struggle to effectively gauge semantic consistency between model outputs and ground truth, and (2) The inherent incompleteness of evaluation benchmarks, primarily due to restrictive human annotation schemas, resulting in underestimated LLM performances. Inspired by the principles in subjective question correction, we propose a new evaluation method, SQC-Score. This method innovatively utilizes LLMs, fine-tuned through subjective question correction data, to refine matching between model outputs and golden labels. Additionally, by incorporating a Natural Language Inference (NLI) model, SQC-Score enriches golden labels, addressing benchmark incompleteness by acknowledging correct yet previously omitted answers. Results on three information extraction tasks show that SQC-Score is more preferred by human annotators than the baseline metrics. Utilizing SQC-Score, we conduct a comprehensive evaluation of the state-of-the-art LLMs and provide insights for future research for information extraction. Dataset and associated codes can be accessed at https://github.com/THU-KEG/SQC-Score.

==> table/3-case-study.tex <==
\begin{table*}[t]
\centering
\begin{tabular}{>{\centering\arraybackslash}m{3.5cm} >{\centering\arraybackslash}m{3cm} >{\centering\arraybackslash}m{1.5cm} >{\centering\arraybackslash}m{1.5cm} >{\centering\arraybackslash}m{1cm} >{\centering\arraybackslash}m{1cm} >{\centering\arraybackslash}m{1cm} >{\centering\arraybackslash}m{1cm} >{\centering\arraybackslash}m{3cm}}
\toprule
\textbf{text} & \textbf{pred} & \textbf{SQC-SCORE-LLAMA2-chat} & \textbf{SQC-SCORE-Tulu} & \textbf{F1-Score} & \textbf{BERT-Score} & \textbf{BART-Score} & \textbf{GPT-Score} & \textbf{gold} \\
\midrule
% Your rows here
India 's oil minister, Mani Shankar Aiyar, on Monday called for China and India to cooperate on energy deals rather than compete as rivals, and talks are planned for this week, news service reports said. & ['India, contains, Mani Shankar Aiyar'] & $100.00$ & $100.00$ & $0.00$ & $53.41$ & $73.06$ & $100.00$ & ['Mani Shankar Aiyar, nationality, India'] \\
\midrule
% Example row 2
The bill, which Hollywood studios have supported enthusiastically, was sponsored by Councilmen David Yassky of Brooklyn and Alan J. Gerson of Manhattan. & ['David Yassky, Councilman representing, Brooklyn'] & $$100.00$$ & $$66.67$$ & $$0.00$$ & $$54.27$$ & $$69.73$$ & $$100.00$$ & ['David Yassky, place\_lived, Brooklyn'] \\

\midrule
After all, New York has often capitulated to corporations threatening to move out of Manhattan by awarding them tax credits, favorable debt financing and property tax abatements to stay put. & ['Manhattan, is\_in, New York'] & $$100.00$$ & $$100.00$$ & $$0.00$$ & $$41.50$$ & $$61.54$$ & $$100.00$$ & ['New York, contains, Manhattan'] \\

\bottomrule
\end{tabular}

\caption{
These are several case studies for SQC-Score. 
For the first and the second cases, the candidate preds are no doubt triples from the given text. However, due to the annotation manual at that time, they are not annotated. Our SQC-Score can capture the drawback of the dataset and remedy this.
For the third case, ['Manhattan, is\_in, New York'] matches ['New York, contains, Manhattan'] because the two triples are nearly the same except their relations. It shows the ability of our SQC-Score to capture simultaneously semantic level in scenarios like structural isomerism and synonym replacement.
From cases above, we can find that since BERTScore and BARTScore are based on the text similarity, they can capture the semantic meaning to some extent but fail to provide a human-like score. Moreover, the dataset incompleteness problem cannot be solved via BERTScore or BARTScore.}
\label{tab:my_label}

\end{table*}


